Planning, Inference and Pragmatics in Sequential Language Games

We study sequential language games in which two players, each with private information, communicate to achieve a common goal. In such games, a successful player must (i) infer the partner's private information from the partner's messages, (ii) generate messages that are most likely to help with the goal, and (iii) reason pragmatically about the partner's strategy. We propose a model that captures all three characteristics and demonstrate their importance in capturing human behavior on a new goal-oriented dataset we collected using crowdsourcing.

==> alphaEffect.tex <==
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
$\alpha$ & 1 & 2 & 5 & 10 & 100\\ \hline
\modelName{} & & & & & \\ \hline
\end{tabular}}
\caption{Effect of $\alpha$ on \modelName{} performance.}
\label{tab:alphaEffect}
\end{table}

==> codalab.tex <==
\paragraph{Reproducibility.} All code, data, and experiments for this
paper are available on the CodaLab platform at
\url{https://worksheets.codalab.org/worksheets/TODO}.


==> dataSetStatistics.tex <==
%\subsection{Dataset Statistics}

\input{data_set_example}
\input{filtered_unfiltered}

We collected a dataset of \gameName{} games on Amazon Mechanical Turk as follows:
200 pairs of players each played all 10 scenarios.
Out of 200 pairs, 32 pairs left the game prematurely which results in 168 pairs playing the total of 1680 games.
Players performed 4967 actions (messages and clicks) total and obtained average score of 7.5 per game.
Interestingly, there is a no significant difference in scores over the 10 scenarios, suggesting that players do not adapt and become more proficient with more game play (\reffig{gamesScoreOverTime}).
\reffig{datasetStatistics} shows the statistics of the collected corpus.
\reffig{datasetExample} shows one of the games,
along with the distribution of messages in the first time step of all games played on this scenario.

% Filtering
To focus on the strategic aspects of \gameName{}, we filtered the dataset to reduce the words in the tail.
Specifically, we keep a game if all its messages
contain at least one of the 12 most frequent words (shown in
\reffig{wordUsage}) or ``yes'' or ``no'';
1259 out 1680 games survived.
\reftab{filteredUnfiltered} compares the statistics between all games and the kept ones.
%\footnote{We could had a table containing these 14 words and ask the players to choose from them.  We found this setup more natural and players do not need to internalize the table therefore, they will get higher scores.}

% PL: use terminology consistently (scenario, time step, game)

% phenomenas in dataset!
%1) pragmatics
%2) inference
%3) planning
%3) context dependency
%4) human bias
%5) noise 
%Some people decide to all the information at once e.g. \spa{square diamond} or \spa{not top}; 
%some people decide to divide the information and say \spa{blue square} or \spa{bottom right}. 
%Along with seeing pragmatics, inference, planning we can see context dependency e.g. some example.
%Is noisy people use ... 
%human bias (e.g. people prefer to start from top left and set the information.





==> firstPagePic.tex <==



==> modelsParameters.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lccc}
\toprule
			&\bf k&\bf f&\bf b\\ \midrule
\modelName{} &	1	&2	&$\infty$\\
\noInfer 	&	1	&2	&1\\
\noPlan 	&	1	&1	&$\infty$\\
\noPrag 	&	0	&2	&$\infty$\\
\bottomrule
\end{tabular}

\caption{\label{tab:modelsParameters} Hyperparameters and the performance of different models on \gameName{}
  (average log-likelihood per message).
Best $\alpha$ shows the value of $\alpha$ that leads to the best performance for that configuration.
%\ndg{these are small differences in LL, and i feel like reviewers won't know how much to trust them. it would be great to have bootstrapped CIs....}
}
\end{table}


==> resultBestModels.tex <==
\begin{figure}[t]
\newcommand{\scc}{0.85}
\centering
\pgfplotsset{mystyle/.style={%   xmax=1.1,xmin=0,
   ymin= -3.9,ymax=-2.8,
%height=2.5in,
   xlabel=\emph{$\alpha$},
ylabel=\emph{average log-likelihood},
    legend pos= south east,
 ymajorgrids=true,
    grid style=dashed,
legend cell align=left,}}

\begin{tikzpicture}[baseline,scale=\scc]

\begin{axis}[mystyle]

\addplot[mark=triangle]
coordinates{
(1,-3.7729)
(4,-3.1947)
(5,-3.1029)
(6,-3.0537)
(7,-3.0046)
(9,-2.937)
(10,-2.9262)
(11,-2.9274)
(15,-2.9538)
(20,-2.991)
(25,-3.0466)
};

\addplot
coordinates{
(1,-3.5893)
(4,-3.2603)
(5,-3.2052)
(6,-3.1617)
(7,-3.128)
(9,-3.0929)
(10,-3.0891)
(11,-3.0906)
(15,-3.1134)
(20,-3.1377)
(25,-3.1558)
};

\addplot
coordinates{
(1,-3.8311)
(4,-3.1335)
(5,-3.0512)
(6,-2.9914)
(7,-2.9486)
(9,-2.9078)
(10,-2.9027)
(11,-2.9028)
(15,-2.9317)
(20,-2.997)
(25,-3.0463)
};

\addplot[color=blue,mark=x]
coordinates{
(1,-3.607)
(4,-3.1104)
(5,-3.0668)
(6,-3.0562)
(7,-3.0613)
(9,-3.0834)
(10,-3.0961)
(11,-3.1096)
(15,-3.1575)
(20,-3.2221)
(25,-3.2901)
};

\legend{
\modelName{},
\noPrag,
\noInfer,
\noPlan
}
\end{axis}\end{tikzpicture}

\caption{Performance of the different models on \gameName{} with different values for $\alpha$.
\modelName{} and \noInfer{} outperforms the other two models.
\noPlan{} has its peak in $\alpha=6$ while the other three have their peaks in $\alpha=10$.
Greater values for $\alpha$ means the model assumes humans are more rational (choose the best actions more aggressively).
}
\label{fig:resultBestModels}
\end{figure}



==> summary.tex <==
\subsection{Summary}
\fk{I think it would be nice if give a summary here and bring Figure 9 here. What do you think?}

==> table_word_frequency.tex <==
\begin{table*}
\scalebox{0.7}{
\begin{tabular}{|l|c|l|c|l|c|l|c|}
\hline
left  & 555 & top  & 499 & square  & 473 & yellow  & 387\\\hline
bottom  & 376 & blue  & 363 & green  & 347 & right  & 330\\\hline
diamond  & 311 & circle  & 285 & middle  & 243 & not  & 170\\\hline
column  & 108 & row  & 103 & one  & 81 & color  & 73\\\hline
two  & 72 & no  & 69 & first  & 59 & squares  & 42\\\hline
three  & 40 & which  & 34 & both  & 32 & what  & 30\\\hline
four  & 30 & shape  & 27 & diamonds  & 25 & side  & 24\\\hline
upper  & 23 & center  & 23 & maybe  & 22 & c  & 21\\\hline	
\end{tabular}}\hspace{0.1cm}%
\scalebox{0.7}{
\begin{tabular}{|l|c|l|c|l|c|l|c|}
\hline
top left  & 146 & bottom left  & 119 & top right  & 113 & yellow square  & 100\\\hline
blue square  & 81 & bottom right  & 69 & yellow diamond  & 63 & blue  & 62\\\hline
green diamond  & 62 & blue circle  & 57 & square diamond  & 55 & green  & 52\\\hline
left column  & 48 & top middle  & 46 & no  & 46 & square  & 46\\\hline
left  & 45 & circle diamond  & 39 & green square  & 38 & yellow  & 37\\\hline
top row  & 36 & circle  & 34 & top  & 33 & green circle  & 31\\\hline
color  & 30 & top bottom  & 29 & blue green  & 28 & yellow green  & 28\\\hline
blue yellow  & 27 & bottom  & 26 & yellow circle  & 25
 & not middle  & 25\\\hline
\end{tabular}}
\end{table*}
